Majority or Minority: Data Imbalance Learning Method for Named Entity Recognition

Data imbalance presents a significant challenge in various machine learning (ML) tasks, particularly named entity recognition (NER) within natural language processing (NLP). NER exhibits a data imbalance with a long-tail distribution, featuring numerous minority classes (i.e., entity classes) and a single majority class (i.e., O-class). This imbalance leads to misclassifications of the entity classes as the O-class. To tackle this issue, we propose a simple and effective learning method named majority or minority (MoM) learning. MoM learning incorporates the loss computed only for samples whose ground truth is the majority class into the loss of the conventional ML model. Evaluation experiments on four NER datasets (Japanese and English) showed that MoM learning improves prediction performance of the minority classes without sacrificing the performance of the majority class and is more effective than widely known and state-of-the-art methods. We also evaluated MoM learning using frameworks as sequential labeling and machine reading comprehension, which are commonly used in NER. Furthermore, MoM learning has achieved consistent performance improvements regardless of language or framework.

==> tables/tex/sentence.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\centering
\caption{Comparison of performance for each entity for baseline and FL and MoM learning using BERT for CoNLL2003 test data in sequential labeling.
This test data was separated by sentence and non-sentence based on the presence or absence of periods.
The prefixes \texttt{B} and \texttt{I} are merged for display purposes; MoM learning outperformed the baseline but was comparable in performance to FL.
}
\label{tab:sentence}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
\multicolumn{7}{c}{\textbf{Sentences}}  \\ \cmidrule(){1-7}
\multicolumn{1}{r}{} & \multicolumn{1}{l}{\texttt{MISC}}  & \multicolumn{1}{l}{\texttt{LOC}}   & \multicolumn{1}{l}{\texttt{ORG}}   & \multicolumn{1}{l}{\texttt{PER}}   & \multicolumn{1}{l}{$\mathcal{O}$} & \multicolumn{1}{l}{\textbf{macro-F1}} \\  \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(l){7-7}
\textbf{BERT}  & 82.50 & 90.98 & 87.45 & 96.29 & 99.54 & 91.35 \\
\textbf{w/ FL} & 84.73 & \textbf{92.53} & 89.48 & \textbf{97.27} & \textbf{99.58} & 92.72 \\
\textbf{w/ MoM} & \textbf{84.88} & 92.46 & \textbf{89.57} & 97.25 & \textbf{99.58} & \textbf{92.75} \\ \toprule
\multicolumn{7}{c}{\textbf{Non-Sentences}}  \\ \cmidrule(){1-7}
\multicolumn{1}{r}{} & \multicolumn{1}{l}{\texttt{MISC}}  & \multicolumn{1}{l}{\texttt{LOC}}   & \multicolumn{1}{l}{\texttt{ORG}}   & \multicolumn{1}{l}{\texttt{PER}}   & \multicolumn{1}{l}{$\mathcal{O}$} & \multicolumn{1}{l}{\textbf{macro-F1}} \\  \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(l){7-7}
\textbf{BERT} & 65.95 & 94.10 & 92.57 & 98.35 & 99.07 & 90.01 \\
\textbf{w/ FL} & \textbf{69.30} & 94.42 & 93.74 & \textbf{98.31} & \textbf{99.22} & \textbf{91.00} \\
\textbf{w/ MoM} & 69.10 & \textbf{94.61} & \textbf{93.93} & 98.14 & 99.20 & \textbf{91.00} \\ \bottomrule
\end{tabular}
% }
\end{table}
